Tell and show: Combining multiple modalities to communicate manipulation tasks to a robot

As human-robot collaboration is becoming more widespread, there is a need for a more natural way of communicating with the robot. This includes combining data from several modalities together with the context of the situation and background knowledge. Current approaches to communication typically rely only on a single modality or are often very rigid and not robust to missing, misaligned, or noisy data. In this paper, we propose a novel method that takes inspiration from sensor fusion approaches to combine uncertain information from multiple modalities and enhance it with situational awareness (e.g., considering object properties or the scene setup). We first evaluate the proposed solution on simulated bimodal datasets (gestures and language) and show by several ablation experiments the importance of various components of the system and its robustness to noisy, missing, or misaligned observations. Then we implement and evaluate the model on the real setup. In human-robot interaction, we must also consider whether the selected action is probable enough to be executed or if we should better query humans for clarification. For these purposes, we enhance our model with adaptive entropy-based thresholding that detects the appropriate thresholds for different types of interaction showing similar performance as fine-tuned fixed thresholds.

==> 8_old_text.tex <==
\section{old text}

--------------------

OLD TEXT 

-----------
\noindent\textbf{General case. } If we don't know which category is which word (i.e., if it is expressing action, object or direction parameter), we have to work with all possible word combinations over the modalities and then determine the most probable action. First, we compute likelihoods that the action $a_j$ is expressed by the given combination of words in sentences from different modalities. This leads to a tensor with $M$ dimensions, each dimension having the size corresponding to the length of the sentence $S^m$. This likelihood tensor for each action $a \in \mathcal{A}$ is computed as follows:

\begin{equation}
\begin{split}
    L_{i_1,...,i_M}(a)=  &\{\Diamond_{m=1}^M\left[W_m*l(\mathcal{C}(\mathbf{w}^m_{i_m})=C_a)*\mathbf{w}^m_{i_m}(j)\right]\} * \\ &\alpha_{a} * \beta_{a}, \\
    &\forall i_1,..,i_M; i_m \in [0,len(\mathbf{S}^m)]
\end{split}
\end{equation}

where $\Diamond$ symbolizes mixing operation (e.g. multiplication, sum or other operator) over the values, the mixing goes over all available modalities $m$ ($M$ is the total number of modalities),  $l(\mathcal{C}(\mathbf{w}^m_{i_m})=C_a)$ is a likelihood that the category of parameter expressed by the word $\mathbf{w}^m_{i_m}$  is $C_a$ (i.e., $\mathbf{w}^m_{i_m}$ is action word), $\mathbf{w}^m_{i_m}(j)$ is likelihood that word $\mathbf{w}^m_{i_m}$ expresses action $a_j$, $W_m$ is the weight of the modality $m$. This term is multiplied by two penalization parameters: $\alpha$ is penalization parameter for not fitting action parameters (see section~\ref{sec:penal_arity}), $\beta$ is the penalization parameter for object features that are not satisfied (see section~\ref{sec:penal_arity}). Please note, that $\mathbf{w}_0^m$ corresponds to the $0$-th word of the sentence $\mathbf{S}^m$, which corresponds to the option that the action is not expressed in the given modality.


\subsection{Merging algorithm - action selection}
We want to determine which action with which parameters is the most probably expressed by human. To do so, we first compute likelihoods for all possible actions and determine the most probable action. We show how to do so both in the general case, where we expect that we don't know which type of parameter is expressed by which word, as well as simplified version for the case that we know for each word which category of parameter it expresses.

\noindent\textbf{General case. } If we don't know which category is which word (i.e., if it is expressing action, object or direction parameter), we have to work with all possible word combinations over the modalities and then determine the most probable action. First, we compute likelihoods that the action $a_j$ is expressed by the given combination of words in sentences from different modalities. This leads to a tensor with $M$ dimensions, each dimension having the size corresponding to the length of the sentence $S^m$. This likelihood tensor for each action $a \in \mathcal{A}$ is computed as follows:

\begin{equation}
\begin{split}
    L_{i_1,...,i_M}(a)=  &\{\Diamond_{m=1}^M\left[W_m*l(\mathcal{C}(\mathbf{w}^m_{i_m})=C_a)*\mathbf{w}^m_{i_m}(j)\right]\} * \\ &\alpha_{a} * \beta_{a}, \\
    &\forall i_1,..,i_M; i_m \in [0,len(\mathbf{S}^m)]
\end{split}
\end{equation}

where $\Diamond$ symbolizes mixing operation (e.g. multiplication, sum or other operator) over the values, the mixing goes over all available modalities $m$ ($M$ is the total number of modalities),  $l(\mathcal{C}(\mathbf{w}^m_{i_m})=C_a)$ is a likelihood that the category of parameter expressed by the word $\mathbf{w}^m_{i_m}$  is $C_a$ (i.e., $\mathbf{w}^m_{i_m}$ is action word), $\mathbf{w}^m_{i_m}(j)$ is likelihood that word $\mathbf{w}^m_{i_m}$ expresses action $a_j$, $W_m$ is the weight of the modality $m$. This term is multiplied by two penalization parameters: $\alpha$ is penalization parameter for not fitting action parameters (see section~\ref{sec:penal_arity}), $\beta$ is the penalization parameter for object features that are not satisfied (see section~\ref{sec:penal_arity}). Please note, that $\mathbf{w}_0^m$ corresponds to the $0$-th word of the sentence $\mathbf{S}^m$, which corresponds to the option that the action is not expressed in the given modality.

Then the most probable action $a_j$ is selected by:

\begin{equation}
    argmax_{j, i_1,..,i_m}(L_{i_1,...,i_m}(a_j))
\end{equation}
We decide to execute this action only if it exceeds the given threshold and has enough difference from other options (see Sec.~\ref{sec:thresholding})


\noindent\textbf{Known categories case.} Given that we for each word know category of the parameter (i.e., we know which word expresses the action), each tensor has only one non-zero value and we can simplify the equation (1) as follows:

\begin{equation}
    l(a)=  &\{\Diamond_{m=1}^M\left(W_m*\mathbf{w}^m_a(j)\right)\} * \alpha_{a} * \beta_{a}, 
\end{equation}
where $w^m_a$ is the word from the modality $m$ that expresses parameter of category $C_a$.


We have sentence $\mathcal{S}$ which includes all information from all recorded modalities ($M$).

Our system has three levels. The first level includes different modality types. We consider speech-language ($\mathcal{S}_L$) converted to written text and ($\mathcal{S}_G$) natural human hand gestures. Gestures are considered an everyday intuitive pseudo-language. Our approach enables us to extend the number of modalities to others, such as body posture, joystick language, and others, but we will stick to the two mentioned ones ($M=2$) because they represent challenges large enough for the merge approaches. When we want to merge information from both modalities, we need to ground the information from both modalities into similar means which we want to compare. 

The second level of our system is called a compare-category type arity ($\mathcal{C}$). In general, we want to mainly compare the target task desired by the user, which when executed should fulfill the user's expectations. Other categories are tied to the selected task. It may be selected objects (e.g. which object to pick), target distance metric (e.g. how far to push the object), or further even number (e.g. how many objects to glue). Each category type consists of Probability Vector in all modalities which we wish to merge. Example probability vector may look like:  $\mathcal{S}_L^{\mathcal{C}=template} = [pick: 1.0, place: 0.0, push: 0.0]$.

The third and final level of the system are properties related to "level 2 items".

The last item in our syst



\subsection{Considered category types}

The main category which we want to merge relates to the verb of the sentence, it is the task or action which the user wishes to execute ($\mathcal{C}_\mathcal{T}$). It spans across various complexity levels. From the most trivial ones (e.g. to \textit{Stop} the correct movement from executing) or the more complex ones (e.g. to clean the table). Other "categories" that we consider comparing are selected objects ($\mathcal{C}_\mathcal{S}$), 
\begin{itemize}
    \item other category types
    \item distance category, direction category, storage category
    \item how to assign the category item into the meaning of the sentence
\end{itemize}
Each modality needs to pre-process the input sentence to classify its items with associated "category" types. Then we obtain a list of apparently independent categories, which we are ready to compare. 
We utilize an NL processor to classify the category items in these boxes in an ordered way.
The true relations are more complex looking like a tree structure.   


\section{Materials and Methods}

